Characterizing and Optimizing EDA Flows for the Cloud

Cloud computing accelerates design space exploration in logic synthesis, and parameter tuning in physical design. However, deploying EDA jobs on the cloud requires EDA teams to deeply understand the characteristics of their jobs in cloud environments. Unfortunately, there has been little to no public information on these characteristics. Thus, in this paper, we formulate the problem of migrating EDA jobs to the cloud. First, we characterize the performance of four main EDA applications, namely: synthesis, placement, routing and static timing analysis. We show that different EDA jobs require different machine configurations. Second, using observations from our characterization, we propose a novel model based on Graph Convolutional Networks to predict the total runtime of a given application on different machine configurations. Our model achieves a prediction accuracy of 87%. Third, we develop a new formulation for optimizing cloud deployments in order to reduce deployment costs while meeting deadline constraints. We present a pseudo-polynomial optimal solution using a multi-choice knapsack mapping that reduces costs by 35.29%.

==> 5related_work.tex <==


On the architectural side, Lin \textit{et. al.} proposed a prototype system design, called Web-EDA, for managing EDA projects on the cloud \cite{web-eda}.
Similarly, Man \textit{et. al.} described a system architecture for small and medium-sized teams aiming to perform IC design and testing on the cloud \cite{cloud-eda}.
Both proposals have been addressing the architecture side of managing EDA assets in a distributed cloud environment.
However, they do not address the computational requirements of the specific EDA jobs.
On the application side, Chen \textit{et. al.} have proposed a cloud-native floorplanning algorithm that takes advantage of the massive cloud scale \cite{floorplanning-cloud}.
More recently, scheduling EDA jobs on distributed environments have also gained interest \cite{nanda2019resource}.
However, this work has been focused on maximizing the utilization of a single cluster, and not on the performance of EDA jobs on multi-tenant virtualized environments.

Our work supports and advances the recent need to move EDA jobs to public cloud environments and offers detailed insights as well as a recipe for EDA teams to maximize the benefit from using the cloud while minimizing the cost.
